Caustic Skeleton & Cosmic Web

We present a general formalism for identifying the caustic structure of an evolving mass distribution in an arbitrary dimensional space. For the class of Hamiltonian fluids the identification corresponds to the classification of singularities in Lagrangian catastrophe theory. Based on this we develop a theoretical framework for the formation of the cosmic web, and specifically those aspects that characterize its unique nature: its complex topological connectivity and multiscale spinal structure of sheetlike membranes, elongated filaments and compact cluster nodes. The present work represents an extension of the work by Arnol'd et al., who classified the caustics for the 1- and 2-dimensional Zel'dovich approximation. His seminal work established the role of emerging singularities in the formation of nonlinear structures in the universe. At the transition from the linear to nonlinear structure evolution, the first complex features emerge at locations where different fluid elements cross to establish multistream regions. The classification and characterization of these mass element foldings can be encapsulated in caustic conditions on the eigenvalue and eigenvector fields of the deformation tensor field. We introduce an alternative and transparent proof for Lagrangian catastrophe theory, and derive the caustic conditions for general Lagrangian fluids, with arbitrary dynamics, including dissipative terms and vorticity. The new proof allows us to describe the full 3-dimensional complexity of the gravitationally evolving cosmic matter field. One of our key findings is the significance of the eigenvector field of the deformation field for outlining the spatial structure of the caustic skeleton. We consider the caustic conditions for the 3-dimensional Zel'dovich approximation, extending earlier work on those for 1- and 2-dimensional fluids towards the full spatial richness of the cosmic web.

==> Arxiv submission Versie 3/Unfoldings.tex <==

\begin{center}
\begin{tikzpicture}
\node (A1) {$A_1$};
\node [right of=A1] (A2) {$A_2$};
\node [right of=A2] (A3) {$A_3$};
\node [right of=A3] (A4) {$A_4$};
\node [right of=A4] (A5) {$A_5$};
\node [right of=A5] (A6) {$A_6$};
\node [right of=A6] (A7) {$A_7$};
\node [right of=A7] (A8) {$A_8$};
\node [right of=A8] (A9) {$A_9$};
\node [right of=A9] (A10) {$\dots$};
\node [below of=A4] (D4) {$D_4$};
\node [below of=A5] (D5) {$D_5$};
\node [below of=A6] (D6) {$D_6$};
\node [below of=A7] (D7) {$D_7$};
\node [below of=A8] (D8) {$D_8$};
\node [below of=A9] (D9) {$A_9$};
\node [below of=A10] (D10) {$\dots$};
\node [below of=D6] (E6) {$E_6$};
\node [below of=D7] (E7) {$E_7$};
\node [below of=D8] (E8) {$E_8$};
  \draw[<-] (A1) to  (A2);
  \draw[<-] (A2) to  (A3);
  \draw[<-] (A3) to  (A4);
  \draw[<-] (A4) to  (A5);
  \draw[<-] (A5) to  (A6);
  \draw[<-] (A6) to  (A7);
  \draw[<-] (A7) to  (A8);
  \draw[<-] (A8) to  (A9);
  \draw[<-] (A9) to  (A10);
  \draw[<-] (D4) to  (D5);
  \draw[<-] (D5) to  (D6);
  \draw[<-] (D6) to  (D7);
  \draw[<-] (D7) to  (D8);
  \draw[<-] (D8) to  (D9);
  \draw[<-] (D9) to  (D10);
  \draw[<-] (E6) to  (E7);
  \draw[<-] (E7) to  (E8);
  \draw[<-] (A3) to  (D4);
  \draw[<-] (A4) to  (D5);
  \draw[<-] (A5) to  (D6);
  \draw[<-] (A6) to  (D7);
  \draw[<-] (A7) to  (D8);
  \draw[<-] (A4) to [out=302,in=152] (E6);
  \draw[<-] (A5) to  (E6);
  \draw[<-] (A5) to [out=302,in=152] (E7);
  \draw[<-] (A6) to  (E7);
  \draw[<-] (A6) to [out=302,in=152] (E8);
  \draw[<-] (A7) to  (E8);
\end{tikzpicture}
\end{center}

==> Arxiv submission Versie 3/UnfoldingsIndexed.tex <==

\begin{center}
\begin{tikzpicture}
\node (O) {};
\node [below of=O] (A1) {$A_1$};
\node [right of=O] (A2) {$A_2^i$};
\node [right of=A2] (A3) {$A_3^i$};
\node [right of=A3] (A4) {$A_4^i$};
\node [right of=A4] (A5) {$A_5^i$};
\node [below of=A4] (D4) {$D_4^{ij}$};
\node [below of=A5] (D5) {$D_5^{ij}$};
\node [below of=D5] (A5p) {$A_5^j$};
\node [below of=D4] (A4p) {$A_4^j$};
\node [left of=A4p] (A3p) {$A_3^j$};
\node [left of=A3p] (A2p) {$A_2^j$};
  \draw[<-] (A1) to  (A2);
  \draw[<-] (A2) to  (A3);
  \draw[<-] (A3) to  (A4);
  \draw[<-] (A4) to  (A5);
  \draw[<-] (D4) to  (D5);
  \draw[<-] (A3) to  (D4);
  \draw[<-] (A4) to  (D5);
  \draw[<-] (A3p) to  (D4);
  \draw[<-] (A4p) to  (D5);
  \draw[<-] (A4p) to (A5p);
  \draw[<-] (A3p) to (A4p);
  \draw[<-] (A2p) to (A3p);
  \draw[<-] (A1) to (A2p);
\end{tikzpicture}
\end{center}

==> Arxiv submission Versie 3/UnfoldingsRes.tex <==

\begin{center}
\begin{tikzpicture}
\node (A1) {$A_1$};
\node [right of=A1] (A2) {$A_2$};
\node [right of=A2] (A3) {$A_3$};
\node [right of=A3] (A4) {$A_4$};
\node [right of=A4] (A5) {$A_5$};
\node [below of=A4] (D4) {$D_4$};
\node [below of=A5] (D5) {$D_5$};
  \draw[<-] (A1) to  (A2);
  \draw[<-] (A2) to  (A3);
  \draw[<-] (A3) to  (A4);
  \draw[<-] (A4) to  (A5);
  \draw[<-] (D4) to  (D5);
  \draw[<-] (A3) to  (D4);
  \draw[<-] (A4) to  (D5);
\end{tikzpicture}
\end{center}
